Affinity CNN: Learning Pixel-Centric Pairwise Relations for Figure/Ground Embedding

Spectral embedding provides a framework for solving perceptual organization problems, including image segmentation and figure/ground organization. From an affinity matrix describing pairwise relationships between pixels, it clusters pixels into regions, and, using a complex-valued extension, orders pixels according to layer. We train a convolutional neural network (CNN) to directly predict the pairwise relationships that define this affinity matrix. Spectral embedding then resolves these predictions into a globally-consistent segmentation and figure/ground organization of the scene. Experiments demonstrate significant benefit to this direct coupling compared to prior works which use explicit intermediate stages, such as edge detection, on the pathway from image to affinities. Our results suggest spectral embedding as a powerful alternative to the conditional random field (CRF)-based globalization schemes typically coupled to deep neural networks.

==> Makefile <==
# Paths to the programs used by this Makefile.
PDFLATEX = pdflatex
CP = cp
RM = rm
GREP = grep
DIFF = diff -q
TOUCH = touch

# Paths to the input and output files.
TEXFILE = affinity-cnn.tex
PDFFILE = affinity-cnn.pdf
TEXINCLUDES =

# Paths to intermediate files that are created by the make process.
# Do not change these.
TEXLOG = $(basename $(TEXFILE)).log
AUXFILE = $(basename $(TEXFILE)).aux
OLDAUXFILE = ".$(AUXFILE).old"

# If this message appears in TEXLOG, we must re-run LaTeX.
RERUNLATEX = "Rerun to get cross-references right"

# The primary target (created by the command "make") is the PDF file.
pdf: $(PDFFILE)

# This rule uses PDFLaTeX to create a PDF file from a LaTeX file.
# Then PDFLaTeX is re-run to resolve references, as necessary.
$(PDFFILE): $(TEXFILE) $(TEXINCLUDES)
	$(TOUCH) $(AUXFILE)
	$(CP) $(AUXFILE) $(OLDAUXFILE)
	$(PDFLATEX) $<
	while $(GREP) -q $(RERUNLATEX) $(TEXLOG); do $(PDFLATEX) $<; done

# This rule cleans out the files made by the make process.
clean:
	$(RM) -f $(AUXFILE) \
                 $(OLDAUXFILE) \
                 $(TEXLOG) \
                 $(PDFFILE)

